Guiding Visual Question Generation

In traditional Visual Question Generation (VQG), most images have multiple concepts (e.g. objects and categories) for which a question could be generated, but models are trained to mimic an arbitrary choice of concept as given in their training data. This makes training difficult and also poses issues for evaluation -- multiple valid questions exist for most images but only one or a few are captured by the human references. We present Guiding Visual Question Generation - a variant of VQG which conditions the question generator on categorical information based on expectations on the type of question and the objects it should explore. We propose two variants: (i) an explicitly guided model that enables an actor (human or automated) to select which objects and categories to generate a question for; and (ii) an implicitly guided model that learns which objects and categories to condition on, based on discrete latent variables. The proposed models are evaluated on an answer-category augmented VQA dataset and our quantitative results show a substantial improvement over the current state of the art (over 9 BLEU-4 increase). Human evaluation validates that guidance helps the generation of questions that are grammatically coherent and relevant to the given image and objects.

==> tables/table-bertscore.tex <==
\begin{table}[t]
\begin{center}
\begin{adjustbox}{width=0.35\textwidth}
\begin{tabular}{@{}l|ccc@{}}
\toprule
    Model      & \multicolumn{1}{c}{P}  & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} \\
    % & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}      & \multicolumn{1}{c}{}    \\ 
    \midrule
    \multicolumn{4}{c}{\texttt{Comparative}}                          \\
    IMVQG (z-path) & 49.7/91.5  & 43.6/90.5     & 46.6/91.0          \\
    IMVQG (t-path) & 47.4/91.1  & 41.8/90.2    & 44.6/90.6       \\
    WBS & 55.6/92.5 & 48.3/91.3      & 51.9/91.9       \\
    \midrule
    \multicolumn{4}{c}{\texttt{Explicit}}                             \\
    image-guided     & \bf 61.1/93.5  & \bf 56.1/92.6 & \bf 58.6/93.0  \\ 
    \midrule
    \multicolumn{4}{c}{\texttt{Implicit}}                             \\
    image-guided   & 57.2/92.8     & 49.8/91.8    & 53.2/92.3  \\ 
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{\red{Results of BertScore on IMVQG, WBS, and our final models. The two scores for each indicate \texttt{rescale-with-baseline} or not.}}
\label{tab:result-bertscore}
\end{center}
\end{table}

==> tables/table-multi.tex <==
\begin{table}[h]
\begin{adjustbox}{width=0.48\textwidth}
\begin{tabular}{@{}l|llllccc@{}}
\toprule
            \multirow{2}{*}{Model}      & \multicolumn{4}{c}{BLEU}                                                                      & \multicolumn{1}{c}{CIDEr} & \multicolumn{1}{c}{METEOR} & \multicolumn{1}{c}{ROUGE} \\ \cmidrule{2-8}
                                                              & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{4} & \multicolumn{1}{c}{}      & \multicolumn{1}{c}{}       & \multicolumn{1}{c}{}      \\ \midrule
    \multicolumn{8}{c}{\texttt{Comparative}}                          \\
 WBS & \textbf{75.6}         & 56.9                  & 44                    & 33.6                  & 45                        & 26.8                       & 66.7                      \\
                              image-only                        &          69.5            &     56.3                  &       44.9                &          34.1             &        34                   &        27.7                    &       60.1                    \\ \midrule
 \multicolumn{8}{c}{\texttt{Implicit}}                             \\
image-category                    & 72.5                  & 57.6                  & 46.1                  & 35.5                  & 46.1                      & 28.8                       & 66.7                      \\
                             image-objects                     & 73                    & 60.6                  & 47.4                  & 36.1                  & 46.4                      & 28.4                       & 66.1                      \\
                             image-guided                    & 72.6                  & \textbf{61.3}         & \textbf{47.5}         & \textbf{36.6}         & \textbf{47.8}             & \textbf{28.9}              & \textbf{66.9}             \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Multiple reference evaluation results.}
\label{tab:result-multi}
\end{table}

==> tables/table-single.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{0.78\linewidth}{!}{
\begin{tabular}{@{}l|llllccllllc@{}}
\toprule
                         \multirow{2}{*}{Model}                                & \multicolumn{4}{c}{BLEU}                                                                      & \multicolumn{1}{c}{CIDEr} & \multicolumn{1}{c}{METEOR} & \multicolumn{1}{c}{ROUGE} & \multicolumn{3}{c}{MSJ} & \multicolumn{1}{c}{BertScore (F1)}
                         \\ \cmidrule{2-12}
                                                        & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{4} & \multicolumn{1}{c}{}      & \multicolumn{1}{c}{}       & \multicolumn{1}{c}{}      & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{4} & \multicolumn{1}{c}{5}
                                            & \multicolumn{1}{c}{}
                                                        \\ \midrule
                                                        \multicolumn{11}{c}{\texttt{Comparative}} \\
 IMVQG (z-path)$^{\dagger}$          & \textbf{50.1}         & 32.3                  & 24.6                  & 16.3                  & 94.3                      & 20.6                       & 39.6                         & 47.2                    &    38.0                   &  31.5                         & 91.0 \\
                         IMVQG (t-path)                  & 47.4                  & 29.0                  & 19.9                  & 14.5                  & 86.0                      & 18.4                       &  38.4                         &  53.8                     &  44.1                     &  37.2                     & 90.6 \\
                             WBS$^{\ddagger}$ & 42.1                  & 22.4                  & 14.1                  & 9.2                   & 60.2                      & 14.9                       & 29.1                      &  63.2                     &  55.7                    &  49.7                    &91.9 \\
                              DBN & 40.7                  & -                  & -                  & -                   & -                      & 22.6                       & -                      & -                     & -                     & -        & -             \\
                              C3VQG & 41.9                  & 22.1                  & 15.0                  & 10.0                   & 46.9                      & 13.6                       & 42.3                      & -                     & -                     & -              & -       \\
                             image-only                        & 25.9                  & 15.9                  & 9.8                  & 5.9                  & 41.4                      & 13.5                       & 27.8                      & 52.2                  & 42.8                  & 36.0              & -      \\ \midrule \midrule
\multicolumn{11}{c}{\texttt{Explicit}}   \\
image-category                    & 40.8                  & 29.9                  & 22.5                  & 17.3                  & 131                       & 20.8                       & 43.0                      & 64.2                  & 55.5                  & 48.8             & -     \\
                              image-objects                     & 34.7                  & 25.0                    & 19.1                  & 15.0                    & 130                       & 19.4                       & 36.9                      & 67.4                  & 59.2                  & 52.7            & -      \\
                              image-guided                     & 46.3                    & \textbf{36.4}         & \textbf{29.5}         & \textbf{24.4}         & \textbf{214}              & \textbf{25.2}                & \textbf{49.0}             & \textbf{71.3}         & \textbf{63.6}         & \textbf{57.3}         &\textbf{93.0} \\ 
                              image-guided-random                     & 23.6                    & 12.1         & 5.75         & 2.39         & 17.6              & 10.8                & 24.2             & 62.3         & 52.6         & 45.0        & - \\ \midrule
\multicolumn{11}{c}{\texttt{Implicit}} \\   
image-category                    & 28.2                  & 17.1                  & 12.1                  & 9.1                   & 50.5                      & 14.0                         & 28.4                      & 51.8                  & 42.9                  & 36.4          & -        \\
                              image-objects                     & 33.0                    & 21.2                  & 16.1                  & 11.2                  & 60.2                      & 15.6                       & 31.4                      & 53.7                  & 45.3                  & 39.1           & -       \\
                             image-guided                    & 33.9                  & 23.5                  & 16.8                  & 12.6                  & 63.6                      & 16.7                       & 33.7                      & 55.8                  & 48.0                    & 41.9              & 92.3    \\ \bottomrule
\end{tabular}
}
\end{center}
\caption{Single reference evaluation results. ``*-guided'' refers to the combination of category and objects. In the explicit variant only, objects refers to the subset of detected objects and caption keywords, filtered on the target QA pair. $^{\dagger}$ indicates an unrealistic inference regime, using answers as input for question generation. $^{\ddagger}$ WBS scores are from single reference evaluation based on the VQA1.0 pre-trained ``Im. + Cap.'' model provided by the authors. 
% Scores in red are not reported by the paper authors, but we run the metrics run on their pre-trained models.
}
\label{tab:result-single}
\end{table*}
